Game Plan: What AI can do for Football, and What Football can do for AI

The rapid progress in artificial intelligence (AI) and machine learning has opened unprecedented analytics possibilities in various team and individual sports, including baseball, basketball, and tennis. More recently, AI techniques have been applied to football, due to a huge increase in data collection by professional teams, increased computational power, and advances in machine learning, with the goal of better addressing new scientific challenges involved in the analysis of both individual players' and coordinated teams' behaviors. The research challenges associated with predictive and prescriptive football analytics require new developments and progress at the intersection of statistical learning, game theory, and computer vision. In this paper, we provide an overarching perspective highlighting how the combination of these fields, in particular, forms a unique microcosm for AI research, while offering mutual benefits for professional teams, spectators, and broadcasters in the years to come. We illustrate that this duality makes football analytics a game changer of tremendous value, in terms of not only changing the game of football itself, but also in terms of what this domain can mean for the field of AI. We review the state-of-the-art and exemplify the types of analysis enabled by combining the aforementioned fields, including illustrative examples of counterfactual analysis using predictive models, and the combination of game-theoretic analysis of penalty kicks with statistical learning of player attributes. We conclude by highlighting envisioned downstream impacts, including possibilities for extensions to other sports (real and virtual).

==> _backed_up_files/_backed_up_natcomms_imports.tex <==
\setcounter{secnumdepth}{0}

\usepackage{xspace}
\usepackage[utf8]{inputenc}
\usepackage[hidelinks]{hyperref}
% \usepackage{subcaption}
\usepackage[labelfont=bf,labelformat=simple,singlelinecheck=off,justification=raggedright]{subcaption}
\DeclareCaptionLabelFormat{bold}{\textbf{#2}}
\captionsetup{subrefformat=bold}


\usepackage{tabularx}
% \usepackage[labelformat=simple]{subcaption}
% \captionsetup{subrefformat=parens} % change to =parens for parenthesis in \subref
\usepackage{graphicx}
\usepackage[super,comma,sort]{natbib}
\usepackage{multirow}
% \usepackage{booktabs}
\usepackage{nicefrac}
\usepackage[margin=1in]{geometry}
% \usepackage{xcolor}
% \usepackage{subfig}
% \usepackage[dvipsnames]{xcolor}
\usepackage{xspace}
\usepackage{nameref}
\usepackage{authblk}
\usepackage{lineno}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{comment}
\usepackage{nameref}
\makeatletter
\AtBeginDocument{%
  \@ifdefinable{\myorg@nameref}{%
    \LetLtxMacro\myorg@nameref\nameref
    \DeclareRobustCommand*{\nameref}[1]{%
      \emph{\myorg@nameref{#1}}%
    }%
  }%
}
\makeatother

%%%%% Color table cells based on value -----------------------------
\usepackage[table]{xcolor}
\usepackage{pgf}
\usepackage{collcell}
\usepackage{booktabs}

% https://tex.stackexchange.com/a/40603 - only color in table body
\usepackage{etoolbox}

\newtoggle{inTableHeader}% Track if still in header of table
\toggletrue{inTableHeader}% Set initial value
\newcommand*{\StartTableHeader}{\global\toggletrue{inTableHeader}}%
\newcommand*{\EndTableHeader}{\global\togglefalse{inTableHeader}}%

\newtheorem{theorem}{Theorem}
\newtheorem{definition}[theorem]{Definition}
% Redefine tabular to initialize \StartTableHeader at start and end
\let\OldTabular\tabular%
\let\OldEndTabular\endtabular%
\renewenvironment{tabular}{\StartTableHeader\OldTabular}{\OldEndTabular\StartTableHeader}%

 %The min, mid and max values and associated colors
\newcommand*{\MinNumber}{0.0}%
\newcommand*{\MidNumber}{0.5} %
\newcommand*{\MaxNumber}{1.0}%
\definecolor{egtaRed}{HTML}{d61f0b}
\definecolor{egtaYellow}{HTML}{fcf560}
\definecolor{egtaGreen}{HTML}{0ec74f}
\definecolor{egtaBlue}{HTML}{34b1eb}

%Apply the diverging gradient macro
\newcommand{\ApplyGradient}[1]{%
  \iftoggle{inTableHeader}{#1}{
    \ifdim #1 pt > \MidNumber pt
        \pgfmathsetmacro{\PercentColor}{max(min(100.0*(#1 - \MidNumber)/(\MaxNumber-\MidNumber),100.0),0.00)} %
          \edef\x{\noexpand\cellcolor{egtaGreen!\PercentColor!white}}\x\textcolor{black}{#1}%
    \else
        \pgfmathsetmacro{\PercentColor}{max(min(100.0*(\MidNumber - #1)/(\MidNumber-\MinNumber),100.0),0.00)} %
      \edef\x{\noexpand\cellcolor{egtaRed!\PercentColor!white}}\x\textcolor{black}{#1}%
    \fi
  }}
\newcolumntype{R}{>{\collectcell\ApplyGradient}r<{\endcollectcell}}

%Apply the monotonic gradient macro
\newcommand{\ApplyGradientMono}[1]{%
  \iftoggle{inTableHeader}{#1}{
    \pgfmathsetmacro{\PercentColor}{max(min(100.0*(#1 - \MinNumber)/(\MaxNumber-\MinNumber),100.0),0.00)} %
      \edef\x{\noexpand\cellcolor{egtaBlue!\PercentColor!white}}\x\textcolor{black}{#1}%
  }}
  
\newcommand{\gamematrix}[6]{
  \begin{tabular}{c} 
    $\begin{array}{c} \\ #1 \\ #2 \end{array} \hspace{0mm}
    \begin{array}{r@{}c@{}c@{}l}
      & #1 & #2 & \\
      \bigg( & \begin{array}{c} #3 \\ #5 \end{array} & \begin{array}{c} #4 \\ #6 \end{array} & \bigg)
    \end{array}$
  \end{tabular}}
  
\newcolumntype{M}{>{\collectcell\ApplyGradientMono}r<{\endcollectcell}}

%%%%% -----------------------------------------------------------

\usepackage{tikz}
\newcommand{\tikzcircle}[2][red,fill=red]{\tikz[baseline=-0.8ex]\draw[#1,radius=#2] (0,0) circle ;}%

\input{math_commands.tex}

\usepackage[capitalise,noabbrev]{cleveref} % must be loaded last
\crefname{equation}{}{} % Do not show 'Eq.' for equations

\newcommand{\gc}[1]{\textbf{\color{red}[#1]}}%General comment
\definecolor{dmblue300}{HTML}{2267EB}
\newcommand{\mv}[1]{\textbf{\color{dmblue300}[MV: #1]}}%Michal
\definecolor{socolor}{rgb}{1.0,0.31,0.0}
\newcommand{\so}[1]{\textbf{\color{socolor}[SO: #1]}}%Shayegan
\newcommand{\pp}[1]{\textbf{\color{orange}[PP: #1]}}%Pol and Pablo
\newcommand{\mg}[1]{\textbf{\color{magenta}[MG: #1]}}%Marta
\newcommand{\kt}[1]{\textbf{\color{purple}[KT: #1]}}%Karl
\newcommand{\hennes}[1]{\textbf{\color{red}[DH: #1]}}%Daniel
\newcommand{\zw}[1]{\textbf{\color{blue}[ZW: #1]}}%Zhe
\newcommand{\pfm}[1]{\textbf{\color{blue}[PM: #1]}}%Paul
\newcommand{\romu}[1]{\textbf{\color{blue}[$\rho\mu$: #1]}}%Romuald
\newcommand{\ag}[1]{\textbf{\color{magenta}[$AG$: #1]}}%Alexandre
\definecolor{darkergreen}{HTML}{20BD46}
\newcommand{\pleasecheck}[1]{\textbf{\color{darkergreen} #1}}%Please check
\newcommand{\adria}[1]{\textbf{\color{blue}[AR: #1]}}%Adria
\newcommand{\pauline}[1]{\textbf{\color{darkergreen}[$PL$: #1]}}%Pauline
\newcommand{\praneet}[1]{\textbf{\color{blue}[PD: #1]}}%Praneet
\newcommand{\ali}[1]{\textbf{\color{orange}[AE: #1]}}%Praneet
\newcommand{\jb}[1]{\textbf{\color{purple}[JB: #1]}}%Jackson
\newcommand{\mr}[1]{\textcolor{blue}{\textbf{[MR: } #1\textbf{]}}}

% Temporarily hide comments
\renewcommand{\mv}[1]{\ignorespaces}
\renewcommand{\so}[1]{\ignorespaces}
\renewcommand{\kt}[1]{\ignorespaces}
\renewcommand{\pp}[1]{\ignorespaces}
\renewcommand{\mg}[1]{\ignorespaces}
\renewcommand{\hennes}[1]{\ignorespaces}
\renewcommand{\zw}[1]{\ignorespaces} 
\renewcommand{\pfm}[1]{\ignorespaces} \renewcommand{\romu}[1]{\ignorespaces} \renewcommand{\pauline}[1]{\ignorespaces} \renewcommand{\adria}[1]{\ignorespaces}
\renewcommand{\praneet}[1]{\ignorespaces} 
\renewcommand{\ali}[1]{\ignorespaces} 
\renewcommand{\mr}[1]{\ignorespaces}


% Frontiers
\newcommand{\frontierOneGTSL}{Frontier~1~(GT\&SL)\xspace}
\newcommand{\frontierTwoSLV}{Frontier~2~(SL\&CV)\xspace}
\newcommand{\frontierThreeGTV}{Frontier~3~(GT\&CV)\xspace}

==> comments_to_editor.tex <==
Dear editor(s),

It is our pleasure to submit our article, ``Game Plan: What AI can do for Football, and What Football can do for AI", to JAIR. Please find below our responses to the questions on the submission page.

1. [Please state in no more than 150 words why your work is important to other researchers in Artificial Intelligence and how they could make use of your results.]

The paper reviews the intersection of game theory, machine learning, and computer vision as novel territory for AI research applied to football analytics, due to unique associated challenges and opportunities enabled by combining these fields for subsequent development of AI techniques. We overview existing work, placing them into context of the SOTA and categorizing them w.r.t. to AI research frontiers spanned by the above three fields. We lay out a clear plan for how this research can tackle the challenges associated with football analytics, based on learning representations, predictive analytics, and human factors, drawing parallels to the formulation of sports analytics as a reinforcement learning problem. We provide illustrative examples highlighting new insights this frontier-driven research brings forth, illustrating empirical game theory augmented with statistical learning-based player summaries for penalty kick analysis, and highlighting the power of statistical learning in the problem of predicting player trajectories using deep reinforcement learning.

2. [Please list 1--3 papers previously published in JAIR that are closest to your work, and explain in no more than 150 words how your work differs from those papers. If you consider no previous articles in JAIR to be sufficiently close to your work, please state this and instead list a previous JAIR publication that has a similar structure to your submission.]

The following JAIR papers are close in content to our work: 

1. ``Training a Multilingual Sportscaster: Using Perceptual Context to Learn Language" (Chen et al., 2010)

2. ``Scheduling Bipartite Tournaments to Minimize Total Travel Distance" (Hoshino \& Kawarabayashi, 2011)

The following JAIR paper has similar in structure to ours:

3.  ``Evolutionary dynamics of multi-agent learning: A survey" (Bloembergen et al., 2015)

The first two papers investigate topics associated with sports analytics, with the first demonstrating a learning-based approach for training commentators for RoboCup soccer games, and the second conducting a theoretical analysis of tournament scheduling for team sports (with an empirical evaluation on both baseball and basketball). In contrast to these works, ours provides an overview of the state-of-the-art in applications of AI research for football analytics at a significantly broader level. Moreover, it provides concrete details on novel opportunities for further developing AI techniques using football analytics as a novel research microcosm. The third paper is similarly structured to ours in that it provides a survey of state-of-the-art literature, but also goes further in providing empirical validations (Section 5) and examples of applications to robotics (Section 6) where, similar to our submission's penalty kick analysis and surrounded discussions, such results were not previously shown in other publications.

3. [If any part of this paper has been previously published or is under review, please state where and explain how the current paper differs. If not, please state "No" as the response.]

No.
